Meeting Uncertain Threats with Feedback

Air and missile defense, naval force protection, and critical-infrastructure security require rapid allocation of scarce effectors against multiple incoming threats when neutralization is uncertain and observed only after a firing round. We formulate this defensive-allocation problem as a Markov decision process in which a commander assigns a fixed amount of effector capacity each round to heterogeneous threats under three operational objectives: minimizing expected threat-clearance time, maximizing the probability of clearance by a deadline, and maximizing effective assignments before a deadline. Rather than expensive full dynamic optimization, we study simple time-oblivious policies suited to fast implementation. Fair allocation, which ignores threat difficulty and spreads fire evenly, is highly effective: it is optimal for all three objectives under homogeneous threats or low-capacity engagements. Moreover, when effector capacity scales at least linearly with the number of threats, its threat-clearance time trails that of the optimal policy by at most a constant number of rounds. We further develop threat-difficulty-aware greedy policies for each objective, including a constant-factor guarantee for effective assignment maximization. Numerically, greedy policies are near-optimal across heterogeneous instances, while fair allocation remains a principled choice when threat difficulties are unknown.

==> tikzdata/salvo_variance/salvo_variance_gap_grid.tex <==
% Auto-generated by make_salvo_variance_plots.py
% Requires \usepgfplotslibrary{groupplots}
\begin{tikzpicture}
\begin{groupplot}[
    group style={group size=3 by 3, horizontal sep=1.0cm, vertical sep=1.0cm},
    width=0.33\textwidth,
    height=0.26\textwidth,
    xlabel={$n$},
    ylabel={Average optimality gap},
    grid=both,
    tick label style={font=\scriptsize},
    label style={font=\small},
    title style={font=\small},
    legend style={font=\scriptsize},
]
\nextgroupplot[title={DTM, Small Var}]
\addplot table[x=n,y=piFA] {tikzdata/salvo_variance/dtm_small_gap.dat};
\addlegendentry{piFA}
\addplot table[x=n,y=piSL] {tikzdata/salvo_variance/dtm_small_gap.dat};
\addlegendentry{piSL}
\addplot table[x=n,y=piEA] {tikzdata/salvo_variance/dtm_small_gap.dat};
\addlegendentry{piEA}
\addplot table[x=n,y=piR] {tikzdata/salvo_variance/dtm_small_gap.dat};
\addlegendentry{piR}
\nextgroupplot[title={DTM, Medium Var}]
\addplot table[x=n,y=piFA] {tikzdata/salvo_variance/dtm_medium_gap.dat};
\addlegendentry{piFA}
\addplot table[x=n,y=piSL] {tikzdata/salvo_variance/dtm_medium_gap.dat};
\addlegendentry{piSL}
\addplot table[x=n,y=piEA] {tikzdata/salvo_variance/dtm_medium_gap.dat};
\addlegendentry{piEA}
\addplot table[x=n,y=piR] {tikzdata/salvo_variance/dtm_medium_gap.dat};
\addlegendentry{piR}
\nextgroupplot[title={DTM, Large Var}]
\addplot table[x=n,y=piFA] {tikzdata/salvo_variance/dtm_large_gap.dat};
\addlegendentry{piFA}
\addplot table[x=n,y=piSL] {tikzdata/salvo_variance/dtm_large_gap.dat};
\addlegendentry{piSL}
\addplot table[x=n,y=piEA] {tikzdata/salvo_variance/dtm_large_gap.dat};
\addlegendentry{piEA}
\addplot table[x=n,y=piR] {tikzdata/salvo_variance/dtm_large_gap.dat};
\addlegendentry{piR}
\nextgroupplot[title={SLM, Small Var}]
\addplot table[x=n,y=piFA] {tikzdata/salvo_variance/slm_small_gap.dat};
\addlegendentry{piFA}
\addplot table[x=n,y=piSL] {tikzdata/salvo_variance/slm_small_gap.dat};
\addlegendentry{piSL}
\addplot table[x=n,y=piEA] {tikzdata/salvo_variance/slm_small_gap.dat};
\addlegendentry{piEA}
\addplot table[x=n,y=piR] {tikzdata/salvo_variance/slm_small_gap.dat};
\addlegendentry{piR}
\nextgroupplot[title={SLM, Medium Var}]
\addplot table[x=n,y=piFA] {tikzdata/salvo_variance/slm_medium_gap.dat};
\addlegendentry{piFA}
\addplot table[x=n,y=piSL] {tikzdata/salvo_variance/slm_medium_gap.dat};
\addlegendentry{piSL}
\addplot table[x=n,y=piEA] {tikzdata/salvo_variance/slm_medium_gap.dat};
\addlegendentry{piEA}
\addplot table[x=n,y=piR] {tikzdata/salvo_variance/slm_medium_gap.dat};
\addlegendentry{piR}
\nextgroupplot[title={SLM, Large Var}]
\addplot table[x=n,y=piFA] {tikzdata/salvo_variance/slm_large_gap.dat};
\addlegendentry{piFA}
\addplot table[x=n,y=piSL] {tikzdata/salvo_variance/slm_large_gap.dat};
\addlegendentry{piSL}
\addplot table[x=n,y=piEA] {tikzdata/salvo_variance/slm_large_gap.dat};
\addlegendentry{piEA}
\addplot table[x=n,y=piR] {tikzdata/salvo_variance/slm_large_gap.dat};
\addlegendentry{piR}
\nextgroupplot[title={EAM, Small Var}]
\addplot table[x=n,y=piFA] {tikzdata/salvo_variance/eam_small_gap.dat};
\addlegendentry{piFA}
\addplot table[x=n,y=piSL] {tikzdata/salvo_variance/eam_small_gap.dat};
\addlegendentry{piSL}
\addplot table[x=n,y=piEA] {tikzdata/salvo_variance/eam_small_gap.dat};
\addlegendentry{piEA}
\addplot table[x=n,y=piR] {tikzdata/salvo_variance/eam_small_gap.dat};
\addlegendentry{piR}
\nextgroupplot[title={EAM, Medium Var}]
\addplot table[x=n,y=piFA] {tikzdata/salvo_variance/eam_medium_gap.dat};
\addlegendentry{piFA}
\addplot table[x=n,y=piSL] {tikzdata/salvo_variance/eam_medium_gap.dat};
\addlegendentry{piSL}
\addplot table[x=n,y=piEA] {tikzdata/salvo_variance/eam_medium_gap.dat};
\addlegendentry{piEA}
\addplot table[x=n,y=piR] {tikzdata/salvo_variance/eam_medium_gap.dat};
\addlegendentry{piR}
\nextgroupplot[title={EAM, Large Var}]
\addplot table[x=n,y=piFA] {tikzdata/salvo_variance/eam_large_gap.dat};
\addlegendentry{piFA}
\addplot table[x=n,y=piSL] {tikzdata/salvo_variance/eam_large_gap.dat};
\addlegendentry{piSL}
\addplot table[x=n,y=piEA] {tikzdata/salvo_variance/eam_large_gap.dat};
\addlegendentry{piEA}
\addplot table[x=n,y=piR] {tikzdata/salvo_variance/eam_large_gap.dat};
\addlegendentry{piR}
\end{groupplot}
\end{tikzpicture}


==> tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_by_cn_with_piFA.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzpicture}

\def\DTMymax{6}

\begin{groupplot}[
    group style={
        group size=3 by 1,
        horizontal sep=1.0cm
    },
    width=0.35\textwidth,
    height=0.30\textwidth,
    xlabel={$n$},
    grid=both,
    tick align=outside,
    xtick pos=bottom,
    ytick pos=left,
    tick label style={font=\scriptsize},
    label style={font=\small},
    title style={font=\small},
    ylabel style={
        align=center,
        at={(axis description cs:-0.36,0.5)},
        anchor=south
    },
    scaled y ticks=false,
    scaled x ticks=false,
    xtick=data,
    xticklabel style={/pgf/number format/fixed},
    ybar,
    /pgf/bar width=1.5pt,
    enlarge x limits=0.18,
    ymin=0,
    ymax=\DTMymax,
    yticklabel style={
        text width=2.0em,
        align=right,
        /pgf/number format/fixed,
        /pgf/number format/precision=1
    },
]

\nextgroupplot[title={$C/n=1$}, ylabel={Avg. perf., DTM}]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};

\nextgroupplot[title={$C/n=2$}]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};

\nextgroupplot[title={$C/n=3$}]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};

\end{groupplot}

\path (group c1r1.south west) -- (group c3r1.south east)
    coordinate[midway] (legendmid);

\matrix[
    matrix of nodes,
    anchor=north,
    row sep=0pt,
    column sep=5pt,
    nodes={anchor=west, inner sep=0pt, outer sep=0pt, font=\footnotesize}
] at ($(legendmid)+(0,-0.9cm)$) {
\tikz{\draw[fill=blue,draw=blue] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{RA}}$ &
\tikz{\draw[fill=orange,draw=orange] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{FA}}$ &
\tikz{\draw[fill=green!60!black,draw=green!60!black] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{SL}}$ &
\tikz{\draw[fill=red,draw=red] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{EA}}$ \\
};

\end{tikzpicture}
\caption{Average DTM objective values for $C/n\in\{1,2,3\}$ under $q_i\sim\mathrm{Unif}(0.05,0.95)$.}
\label{fig:sim_uniform_q005_095_tau3_dtm_by_cn}
\end{figure}


==> tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_obj_by_cn_with_piFA.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzpicture}

% Common y-axis ranges within each row
\def\DTMymax{150}
\def\SLMymax{1}
\def\EAMymax{120}

\begin{groupplot}[
    group style={group size=3 by 3, horizontal sep=1.0cm, vertical sep=1.1cm},
    width=0.35\textwidth,
    height=0.30\textwidth,
    xlabel={$n$},
    grid=both,
    tick align=outside,
    xtick pos=bottom,
    ytick pos=left,
    tick label style={font=\scriptsize},
    label style={font=\small},
    title style={font=\small},
    ylabel style={align=center, at={(axis description cs:-0.36,0.5)}, anchor=south},
    scaled y ticks=false,
    scaled x ticks=false,
    xtick=data,
    xticklabel style={/pgf/number format/fixed},
    ybar,
    /pgf/bar width=1.5pt,
    enlarge x limits=0.18,
]

% =========================
% Row 1: DTM
% =========================
\nextgroupplot[
    title={$C/n=1$},
    ylabel={Avg. perf., DTM},
    ymin=0,
    ymax=\DTMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};

\nextgroupplot[
    title={$C/n=2$},
    ymin=0,
    ymax=\DTMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};

\nextgroupplot[
    title={$C/n=3$},
    ymin=0,
    ymax=\DTMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};

% =========================
% Row 2: SLM
% =========================
\nextgroupplot[
    ylabel={Avg. perf., SLM},
    ymin=0,
    ymax=\SLMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn1_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn1_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn1_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn1_obj.dat};

\nextgroupplot[
    ymin=0,
    ymax=\SLMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn2_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn2_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn2_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn2_obj.dat};

\nextgroupplot[
    ymin=0,
    ymax=\SLMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn3_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn3_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn3_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn3_obj.dat};

% =========================
% Row 3: EAM
% =========================
\nextgroupplot[
    ylabel={Avg. perf., EAM},
    xlabel={$n$},
    ymin=0,
    ymax=\EAMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-4pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn1_obj.dat};
\addplot+[bar shift=-2pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn1_obj.dat};
\addplot+[bar shift=0pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn1_obj.dat};
\addplot+[bar shift=2pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn1_obj.dat};
\addplot+[bar shift=4pt, fill=purple, draw=purple]
table[x=n,y=piR] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn1_obj.dat};

\nextgroupplot[
    xlabel={$n$},
    ymin=0,
    ymax=\EAMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-4pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn2_obj.dat};
\addplot+[bar shift=-2pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn2_obj.dat};
\addplot+[bar shift=0pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn2_obj.dat};
\addplot+[bar shift=2pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn2_obj.dat};
\addplot+[bar shift=4pt, fill=purple, draw=purple]
table[x=n,y=piR] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn2_obj.dat};

\nextgroupplot[
    xlabel={$n$},
    ymin=0,
    ymax=\EAMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-4pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn3_obj.dat};
\addplot+[bar shift=-2pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn3_obj.dat};
\addplot+[bar shift=0pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn3_obj.dat};
\addplot+[bar shift=2pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn3_obj.dat};
\addplot+[bar shift=4pt, fill=purple, draw=purple]
table[x=n,y=piR] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn3_obj.dat};

\end{groupplot}

\path (group c1r3.south west) -- (group c3r3.south east)
    coordinate[midway] (legendmid);

\matrix[
    matrix of nodes,
    anchor=north,
    row sep=2pt,
    column sep=4pt,
    nodes={anchor=west, inner sep=0pt, outer sep=0pt, font=\footnotesize}
] at ($(legendmid)+(0,-0.95cm)$) {
\tikz{\draw[fill=blue,draw=blue] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{RA}}$ &
\tikz{\draw[fill=orange,draw=orange] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{FA}}$ &
\tikz{\draw[fill=green!60!black,draw=green!60!black] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{SL}}$ \\
\tikz{\draw[fill=red,draw=red] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{EA}}$ &
\tikz{\draw[fill=purple,draw=purple] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{R}}$ & & \\
};

\end{tikzpicture}
\caption{Average objective values under DTM, SLM, and EAM for fixed $\tau=3$ and capacity ratios $C/n\in\{1,2,3\}$. Each row corresponds to one objective, and each column corresponds to one value of $C/n$.}
\label{fig:sim_uniform_q005_095_tau3_obj_by_cn}
\end{figure}


==> tikzdata/simulation_uniform_q_005_095_tau5/sim_uniform_q005_095_tau5_dtm_by_cn_with_piFA.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzpicture}

\def\DTMymax{6}

\begin{groupplot}[
    group style={
        group size=3 by 1,
        horizontal sep=1.0cm
    },
    width=0.35\textwidth,
    height=0.30\textwidth,
    xlabel={$n$},
    grid=both,
    tick align=outside,
    xtick pos=bottom,
    ytick pos=left,
    tick label style={font=\scriptsize},
    label style={font=\small},
    title style={font=\small},
    ylabel style={
        align=center,
        at={(axis description cs:-0.36,0.5)},
        anchor=south
    },
    scaled y ticks=false,
    scaled x ticks=false,
    xtick=data,
    xticklabel style={/pgf/number format/fixed},
    ybar,
    /pgf/bar width=1.5pt,
    enlarge x limits=0.18,
    ymin=0,
    ymax=\DTMymax,
    yticklabel style={
        text width=2.0em,
        align=right,
        /pgf/number format/fixed,
        /pgf/number format/precision=1
    },
]

\nextgroupplot[title={$C/n=1$}, ylabel={Avg. perf., DTM}]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};

\nextgroupplot[title={$C/n=2$}]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};

\nextgroupplot[title={$C/n=3$}]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};

\end{groupplot}

\path (group c1r1.south west) -- (group c3r1.south east)
    coordinate[midway] (legendmid);

\matrix[
    matrix of nodes,
    anchor=north,
    row sep=0pt,
    column sep=5pt,
    nodes={anchor=west, inner sep=0pt, outer sep=0pt, font=\footnotesize}
] at ($(legendmid)+(0,-0.9cm)$) {
\tikz{\draw[fill=blue,draw=blue] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{RA}}$ &
\tikz{\draw[fill=orange,draw=orange] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{FA}}$ &
\tikz{\draw[fill=green!60!black,draw=green!60!black] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{SL}}$ &
\tikz{\draw[fill=red,draw=red] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{EA}}$ \\
};

\end{tikzpicture}
\caption{Average DTM objective values for $C/n\in\{1,2,3\}$ under $q_i\sim\mathrm{Unif}(0.05,0.95)$.}
\label{fig:sim_uniform_q005_095_tau3_dtm_by_cn}
\end{figure}


==> tikzdata/simulation_uniform_q_005_095_tau5/sim_uniform_q005_095_tau5_obj_by_cn_with_piFA.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzpicture}

% Common y-axis ranges within each row
\def\DTMymax{150}
\def\SLMymax{1}
\def\EAMymax{120}

\begin{groupplot}[
    group style={group size=3 by 3, horizontal sep=1.0cm, vertical sep=1.1cm},
    width=0.35\textwidth,
    height=0.30\textwidth,
    xlabel={$n$},
    grid=both,
    tick align=outside,
    xtick pos=bottom,
    ytick pos=left,
    tick label style={font=\scriptsize},
    label style={font=\small},
    title style={font=\small},
    ylabel style={align=center, at={(axis description cs:-0.36,0.5)}, anchor=south},
    scaled y ticks=false,
    scaled x ticks=false,
    xtick=data,
    xticklabel style={/pgf/number format/fixed},
    ybar,
    /pgf/bar width=1.5pt,
    enlarge x limits=0.18,
]

% =========================
% Row 1: DTM
% =========================
\nextgroupplot[
    title={$C/n=1$},
    ylabel={Avg. perf., DTM},
    ymin=0,
    ymax=\DTMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn1_obj.dat};

\nextgroupplot[
    title={$C/n=2$},
    ymin=0,
    ymax=\DTMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn2_obj.dat};

\nextgroupplot[
    title={$C/n=3$},
    ymin=0,
    ymax=\DTMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_dtm_cn3_obj.dat};

% =========================
% Row 2: SLM
% =========================
\nextgroupplot[
    ylabel={Avg. perf., SLM},
    ymin=0,
    ymax=\SLMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn1_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn1_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn1_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn1_obj.dat};

\nextgroupplot[
    ymin=0,
    ymax=\SLMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn2_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn2_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn2_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn2_obj.dat};

\nextgroupplot[
    ymin=0,
    ymax=\SLMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-3pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn3_obj.dat};
\addplot+[bar shift=-1pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn3_obj.dat};
\addplot+[bar shift=1pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn3_obj.dat};
\addplot+[bar shift=3pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_slm_cn3_obj.dat};

% =========================
% Row 3: EAM
% =========================
\nextgroupplot[
    ylabel={Avg. perf., EAM},
    xlabel={$n$},
    ymin=0,
    ymax=\EAMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-4pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn1_obj.dat};
\addplot+[bar shift=-2pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn1_obj.dat};
\addplot+[bar shift=0pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn1_obj.dat};
\addplot+[bar shift=2pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn1_obj.dat};
\addplot+[bar shift=4pt, fill=purple, draw=purple]
table[x=n,y=piR] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn1_obj.dat};

\nextgroupplot[
    xlabel={$n$},
    ymin=0,
    ymax=\EAMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-4pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn2_obj.dat};
\addplot+[bar shift=-2pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn2_obj.dat};
\addplot+[bar shift=0pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn2_obj.dat};
\addplot+[bar shift=2pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn2_obj.dat};
\addplot+[bar shift=4pt, fill=purple, draw=purple]
table[x=n,y=piR] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn2_obj.dat};

\nextgroupplot[
    xlabel={$n$},
    ymin=0,
    ymax=\EAMymax,
    yticklabel style={text width=2.0em, align=right, /pgf/number format/fixed, /pgf/number format/precision=1}
]
\addplot+[bar shift=-4pt, fill=blue, draw=blue]
table[x=n,y=piRA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn3_obj.dat};
\addplot+[bar shift=-2pt, fill=orange, draw=orange]
table[x=n,y=piFA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn3_obj.dat};
\addplot+[bar shift=0pt, fill=green!60!black, draw=green!60!black]
table[x=n,y=piSL] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn3_obj.dat};
\addplot+[bar shift=2pt, fill=red, draw=red]
table[x=n,y=piEA] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn3_obj.dat};
\addplot+[bar shift=4pt, fill=purple, draw=purple]
table[x=n,y=piR] {tikzdata/simulation_uniform_q_005_095_tau3/sim_uniform_q005_095_tau3_eam_cn3_obj.dat};

\end{groupplot}

\path (group c1r3.south west) -- (group c3r3.south east)
    coordinate[midway] (legendmid);

\matrix[
    matrix of nodes,
    anchor=north,
    row sep=2pt,
    column sep=4pt,
    nodes={anchor=west, inner sep=0pt, outer sep=0pt, font=\footnotesize}
] at ($(legendmid)+(0,-0.95cm)$) {
\tikz{\draw[fill=blue,draw=blue] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{RA}}$ &
\tikz{\draw[fill=orange,draw=orange] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{FA}}$ &
\tikz{\draw[fill=green!60!black,draw=green!60!black] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{SL}}$ \\
\tikz{\draw[fill=red,draw=red] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{EA}}$ &
\tikz{\draw[fill=purple,draw=purple] (0,0) rectangle (0.16,0.10);} &
$\pi_{\textsf{R}}$ & & \\
};

\end{tikzpicture}
\caption{Average objective values under DTM, SLM, and EAM for fixed $\tau=3$ and capacity ratios $C/n\in\{1,2,3\}$. Each row corresponds to one objective, and each column corresponds to one value of $C/n$.}
\label{fig:sim_uniform_q005_095_tau3_obj_by_cn}
\end{figure}

